Diagnostics of cognitive failures in multi-agent expert systems using dynamic evaluation protocols and subsequent mutation of the processing context

The rapid evolution of neural architectures - from multilayer perceptrons to large-scale Transformer-based models - has enabled language models (LLMs) to exhibit emergent agentic behaviours when equipped with memory, planning, and external tool use. However, their inherent stochasticity and multi-step decision processes render classical evaluation methods inadequate for diagnosing agentic performance. This work introduces a diagnostic framework for expert systems that not only evaluates but also facilitates the transfer of expert behaviour into LLM-powered agents. The framework integrates (i) curated golden datasets of expert annotations, (ii) silver datasets generated through controlled behavioural mutation, and (iii) an LLM-based Agent Judge that scores and prescribes targeted improvements. These prescriptions are embedded into a vectorized recommendation map, allowing expert interventions to propagate as reusable improvement trajectories across multiple system instances. We demonstrate the framework on a multi-agent recruiter-assistant system, showing that it uncovers latent cognitive failures - such as biased phrasing, extraction drift, and tool misrouting - while simultaneously steering agents toward expert-level reasoning and style. The results establish a foundation for standardized, reproducible expert behaviour transfer in stochastic, tool-augmented LLM agents, moving beyond static evaluation to active expert system refinement.

==> chapters/Bib.tex <==
\section*{Bibliography}

\begin{itemize}
  % related work
  \item Yehudai \textit{et al.} (2025). \textit{Survey on Evaluation of LLM-based Agents: First Systematic Survey}. arXiv preprint arXiv:2503.16416.
  \item Qin \textit{et al.} (2023). \textit{API-Bank: A Comprehensive Benchmark for Tool-Augmented LLMs}. arXiv preprint arXiv:2304.08244.
  \item Song \textit{et al.} (2023). \textit{RestBench: Connecting Large Language Models with Real-World RESTful APIs}. arXiv preprint arXiv:2306.06624.
  \item Zhong \textit{et al.} (2025). \textit{ComplexFuncBench: Exploring Multi-Step and Constrained Function Calling under Long-Context Scenario}. arXiv preprint arXiv:2501.10132.
  \item Li \textit{et al.} (2024). \textit{Reflection-Bench: Probing AI Intelligence with Reflection}. arXiv preprint arXiv:2410.16270.
  \item Huet \textit{et al.} (2025). \textit{Episodic Memories Generation and Evaluation Benchmark for Large Language Models}. arXiv preprint arXiv:2501.13121.
  \item Zhuge \textit{et al.} (2024). \textit{Agent-as-a-Judge: Evaluate Agents with Agents}. arXiv preprint arXiv:2410.10934.
  \item Qi \textit{et al.} (2025). \textit{AGENTIF: Benchmarking Instruction Following of Large Language Models in Agentic Scenarios}. arXiv preprint arXiv:2505.16944.
  \item Zhao \textit{et al.} (2024). \textit{AgentUnit: Unit-Test-Style Evaluation of LLM Agents}. arXiv preprint arXiv:2411.13768.
  \item Kumar \textit{et al.} (2025). \textit{Test4LLM: Automatic Unit Test Generation for LLMs}. arXiv preprint arXiv:2411.13768.
  % intro 
  \item Vaswani \textit{et al.} (2017). \textit{Attention Is All You Need}. In \textit{Advances in Neural Information Processing Systems}. arXiv preprint arXiv:1706.03762.
  \item Brown \textit{et al.} (2020). \textit{Language Models Are Few-Shot Learners}. In \textit{Advances in Neural Information Processing Systems}. arXiv preprint arXiv:2005.14165.
  \item Yao \textit{et al.} (2022). \textit{ReAct: Synergizing Reasoning and Acting in Language Models}. arXiv preprint arXiv:2210.03629.
  \item Schick \textit{et al.} (2023). \textit{Toolformer: Language Models Can Teach Themselves to Use Tools}. arXiv preprint arXiv:2302.04761.
  \item Wu \textit{et al.} (2023). \textit{AutoGen: Enabling Next-Gen LLM Applications via Multi-Agent Conversation}. arXiv preprint arXiv:2308.08155.
% Historical Development of LLMs
  \item Rumelhart, Hinton \& Williams (1986). \textit{Learning representations by back-propagating errors}. Nature 323(6088):533–536.
  \item Hochreiter \& Schmidhuber (1997). \textit{Long Short-Term Memory}. Neural Computation 9(8):1735–1780.
  \item Bahdanau, Cho \& Bengio (2015). \textit{Neural Machine Translation by Jointly Learning to Align and Translate}. In International Conference on Learning Representations (ICLR) 2015. arXiv preprint arXiv:1409.0473.
  \item Radford, Narasimhan, Salimans \& Sutskever (2018). \textit{Improving Language Understanding by Generative Pre-Training}. OpenAI Technical Report, 2018.
  \item Radford, Wu, Child, Luan, Amodei \& Sutskever (2019). \textit{Language Models are Unsupervised Multitask Learners}. OpenAI Technical Report, 2019.
 % Transformer Advancements and GPT Evolution
  \item Xiong \textit{et al.} (2023). \textit{Pre-RMSNorm and Pre-CRMSNorm Transformers}. arXiv preprint arXiv:2305.14858.
  \item Shazeer (2020). \textit{GLU Variants Improve Transformer}. arXiv preprint arXiv:2002.05202.
  \item Su, Lu, Pan \textit{et al.} (2021). \textit{RoFormer: Enhanced Transformer with Rotary Position Embedding}. arXiv preprint arXiv:2104.09864.
  \item Ainslie \textit{et al.} (2023). \textit{GQA: Training Generalized Multi-Query Transformer Models from Multi-Head Checkpoints}. arXiv preprint arXiv:2305.13245.
  \item Touvron \textit{et al.} (2023). \textit{Llama 2: Open Foundation and Fine-Tuned Chat Models}. arXiv preprint arXiv:2307.09288.
  \item Beltagy, Peters \& Cohan (2020). \textit{Longformer: The Long-Document Transformer}. arXiv preprint arXiv:2004.05150.
  \item Li \textit{et al.} (2021). \textit{Position Masking for Improved Layout-Aware Document Understanding}. In Proceedings of ICDAR 2021.
  \item Xiong \textit{et al.} (2020). \textit{On Layer Normalization in the Transformer Architecture}. In International Conference on Learning Representations (ICLR) 2020.
  \item Shazeer \textit{et al.} (2017). \textit{Outrageously Large Neural Networks: The Sparsely-Gated Mixture-of-Experts Layer}. In International Conference on Learning Representations (ICLR) 2017.
  \item Liu \textit{et al.} (2025). \textit{VRoPE: Rotary Position Embedding for Video Large Language Models}. arXiv preprint arXiv:2502.11664.
   % instructGPT
   \item Ouyang \textit{et al.} (2022). \textit{Training Language Models to Follow Instructions with Human Feedback}. In Advances in Neural Information Processing Systems (NeurIPS) 2022. arXiv preprint arXiv:2203.02155.
   % Chain of Thought
  \item Wei \textit{et al.} (2022). \textit{Chain-of-Thought Prompting Elicits Reasoning in Large Language Models}. arXiv preprint arXiv:2201.11903.
  \item Kojima \textit{et al.} (2022). \textit{Large Language Models are Zero-Shot Reasoners}. arXiv preprint arXiv:2205.11916.
  \item Zhang \textit{et al.} (2022). \textit{Automatic Chain of Thought Prompting in Large Language Models}. arXiv preprint arXiv:2210.03493.
  \item Wang \textit{et al.} (2022). \textit{Self-Consistency Improves Chain of Thought Reasoning in Language Models}. arXiv preprint arXiv:2203.11171; In International Conference on Learning Representations (ICLR) 2023.
  \item Yao \textit{et al.} (2023). \textit{Tree of Thoughts: Deliberate Problem Solving with Large Language Models}. arXiv preprint arXiv:2305.10601; In Advances in Neural Information Processing Systems (NeurIPS) 2023
  % DeepSeek
  \item Liu \textit{et al.} (2024). \textit{DeepSeek-V2: A Strong, Economical, and Efficient Mixture-of-Experts Language Model}. arXiv preprint arXiv:2405.04434.
  % Agenic Systems
  \item Shen \textit{et al.} (2023). \textit{HuggingGPT: Solving AI Tasks with ChatGPT and Its Friends in Hugging Face}. arXiv preprint arXiv:2303.17580.
  \item Patil \textit{et al.} (2023). \textit{Gorilla: Large Language Model Connected with Massive APIs}. arXiv preprint arXiv:2305.15334.
  \item Richards (2023). \textit{AutoGPT}. GitHub repository Significant-Gravitas/AutoGPT (initial release Mar 30 2023).
  % Evaluation Back
  \item Papineni \textit{et al.} (2002). \textit{BLEU: a Method for Automatic Evaluation of Machine Translation}. In Proceedings of the 40th Annual Meeting of the Association for Computational Linguistics (ACL), pages 311–318, Philadelphia, PA.
  \item Lin (2004). \textit{ROUGE: A Package for Automatic Evaluation of Summaries}. In Text Summarization Branches Out (ACL Workshop), pages 74–81, Barcelona, Spain.
  \item Hendrycks \textit{et al.} (2021). \textit{Measuring Massive Multitask Language Understanding}. In Proceedings of the International Conference on Learning Representations (ICLR).
  \item Bommasani, Liang \& Lee (2022). \textit{Holistic Evaluation of Language Models (HELM)}. arXiv preprint arXiv:2211.09110.
  \item Lin \textit{et al.} (2022). \textit{TruthfulQA: Measuring How Models Mimic Human Falsehoods}. In Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (ACL), pages 3214–3252.
  \item Srivastava \textit{et al.} (2022). \textit{Beyond the Imitation Game: Quantifying and Extrapolating the Capabilities of Language Models}. arXiv preprint arXiv:2206.04615.
\end{itemize}


==> chapters/background_old.tex <==
\section{Early Neural Language Models: From MLPs to LSTMs}

LLM-based agent systems are stochastic and can behave unpredictably. To operate them reliably, understand the diagnostics introduced in Chapter 3, or devise new methodologies, the reader must have a clear view of the system’s components and how they interact. This chapter provides that foundation. The chapter establishes terminology, assumptions, and evaluation context for Chapter 3: Methodology, including the Agent Diagnostic Method for Expert Systems (ADM–ES), the Text Block Extraction Diagnostic (ED), the Behaviour Diagnostic (BD), and the agent Mutator with its acceptance checks (e.g., mean BERTScore over k). It thereby provides the conceptual baseline needed to interpret results and reproduce procedures in subsequent chapters.

The evolution of large language models (LLMs) is rooted in breakthroughs in neural network design and training strategies that have progressively enabled richer representations, longer context modeling, and more powerful generative capabilities. The journey begins with multilayer perceptrons (MLPs), which demonstrated that layered networks of simple nonlinear units could learn complex input–output mappings through the backpropagation algorithm (Rumelhart et al., 1986). Although these early networks excelled at pattern recognition tasks, they operated on fixed-size inputs and lacked any mechanism to capture sequential dependencies or memory of previous inputs.

To address sequence modeling, researchers developed recurrent neural networks (RNNs), which introduce a hidden state that updates dynamically as new inputs arrive. By maintaining and modifying an internal memory, RNNs could, in principle, remember information from earlier in a sequence. However, practical training of RNNs suffered from vanishing or exploding gradients, making it difficult to learn dependencies spanning more than a few time steps.

The Long Short-Term Memory (LSTM) architecture, introduced by Hochreiter and Schmidhuber (1997), overcame these training challenges by incorporating gating mechanisms—specifically, input, forget, and output gates—that regulate the flow of information into and out of the cell state. This design enabled robust learning of long-range dependencies, and LSTMs rapidly became the backbone of state-of-the-art systems in language modeling, machine translation, and other sequential tasks.

Despite these advances, RNN-based approaches still processed sequence elements in a largely linear, step-by-step fashion. The introduction of attention mechanisms by Bahdanau, Cho, and Bengio (2015) marked a pivotal shift: instead of compressing an entire sequence into a fixed-size vector, attention allows the model to compute a context-dependent weighted sum of all encoder hidden states at each decoding step. This dynamic focus mechanism led to significant improvements in translation quality and opened the door to architectures that rely less on recurrence.

Building on the power of attention, Vaswani \textit{et al.} (2017) proposed the Transformer architecture (Figure \ref{fig:transformer}) in the landmark paper “Attention Is All You Need.” By stacking multi-head self-attention layers interleaved with position-wise feedforward networks, the Transformer dispensed with recurrence entirely. Each token in the input attends to every other token in parallel, enabling both efficient GPU utilization and effective modeling of long-range dependencies. Positional encodings were introduced to inject sequence order information, ensuring that the model remained sensitive to word order despite its parallel structure.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/attention.png}
    \caption{ The Transformer - model architecture}
    \label{fig:transformer}
\end{figure}

The GPT series adapted the Transformer into a decoder-only format optimized for generative pre-training. GPT-1 demonstrated that a unidirectional Transformer, pre-trained on a large corpus and then fine-tuned on task-specific data, could achieve strong performance across multiple benchmarks (Radford et al., 2018). GPT-2 scaled this idea by increasing model size and training data, yielding emergent few-shot learning abilities without task-specific fine-tuning (Radford et al., 2019). GPT-3 further amplified scale—using 175 billion parameters—and showed that in-context learning alone could lead to high-quality performance on tasks ranging from question answering to code generation (Brown et al., 2020).

In each of these stages, improvements in model architecture, training regimes, and scale have collectively enhanced the ability of LLMs to generate coherent, contextually appropriate text. These foundational innovations set the stage for the subsequent emergence of agentic systems, where LLMs are no longer confined to single-turn generation but instead engage in multi-step planning, tool use, and interactive behaviors that reflect increasingly complex, autonomous capabilities.


\section{The Transformer Revolution and the GPT Lineage}

Since the debut of the original GPT decoder‐only model, a series of architectural and training refinements have steadily improved both the efficiency and capabilities of large language models. We organize these innovations into five “steps” of evolution:

\begin{enumerate}[label=\textbf{Step \arabic*:}, leftmargin=*, align=left]
  \item \textbf{Foundation – GPT Decoder Architecture.}  
    The GPT series (Radford et al., 2018; Radford et al., 2019; Brown et al., 2020) introduced the notion that a unidirectional (“causal”) Transformer decoder, pre‐trained on massive text corpora via next‐token prediction, could serve as a general-purpose language engine. Unlike the encoder–decoder setup of the original Transformer, the GPT decoder stacks masked self‐attention layers followed by position‐wise feed-forward networks, enabling autoregressive generation without the need for explicit encoder outputs. This simple yet powerful design demonstrated that, with sufficient scale, language models could perform downstream tasks through zero- and few-shot prompting alone.

  \item \textbf{Alignment via Reinforcement Learning.}  
    With GPT’s generative prowess came concerns over unaligned or unsafe outputs. Reinforcement Learning from Human Feedback (RLHF) (Ouyang et al., 2022) addressed this by treating the language model as a policy in a reinforcement learning framework. Human raters first score model outputs for desired qualities; these scores train a reward model, which in turn guides policy updates via Proximal Policy Optimization. RLHF elevated the “human-likeness” and safety of LLM responses, becoming standard in instruct-tuned variants like InstructGPT and ChatGPT.

  \item \textbf{Accuracy Optimizations.}  
    As models scaled, small architectural tweaks yielded outsized gains in stability and performance:
    \begin{itemize}
      \item \textbf{RMSNorm.} Unlike LayerNorm, which relies on both mean and variance, Root Mean Square normalization (RMSNorm) scales activations solely by their root mean square. This reduces computational overhead and mitigates exploding gradients when training on extremely large datasets or with large batch sizes.
      \item \textbf{SwiGLU Activation.} Replacing the standard GeLU or ReLU in feed-forward blocks, the SwiGLU function gates half the hidden units using a sigmoid, enabling more expressive, conditional computation in the MLP sub-layers without significantly increasing parameter count.
      \item \textbf{RoPE (Rotary Positional Encoding).} Traditional absolute positional encodings can struggle with generalizing to longer sequences. Rotary Positional Encoding injects relative positional information via rotation matrices applied to query/key projections, yielding better extrapolation to unseen sequence lengths and improved accuracy on long-context tasks.
    \end{itemize}

  \item \textbf{Training Efficiency.}  
    To reduce compute without sacrificing quality:
    \begin{itemize}
      \item \textbf{Grouped-Query Attention (GQA).} GQA clusters attention heads into small groups (e.g., eight heads per group), sharing key and value projections within each group. This design cuts computation by 6–8× with only a minor (10–20\%) impact on perplexity, making larger models more practical to deploy.
      \item \textbf{Ghost Attention.} For conversational agents, maintaining a persistent “system” prompt or persona over long dialogues is critical. Ghost Attention passes a lightweight version of the system token through each block as a “ghost,” ensuring core instructions remain salient even after thousands of tokens of user and assistant history.
    \end{itemize}

  \item \textbf{Scaling and Advanced Optimizations.}  
    As context lengths and model sizes grew, new techniques preserved performance and efficiency:
    \begin{itemize}
      \item \textbf{Ultra-Long Context Windows.} Methods like sliding-window attention, chunked processing, and sparse global attention enable models to process tens or hundreds of thousands of tokens in a single pass, critical for document-level understanding and multi-document reasoning.
      \item \textbf{Document-Aware Masking.} During pre-training, isolating attention to within-document token groups prevents the model from conflating patterns across separate documents, improving coherence on multi-text corpora.
      \item \textbf{Document-Level Pre-Norm + SwiGLU Decoder.} Applying layer normalization before attention and feed-forward sub-layers (pre-norm) on document chunks, combined with SwiGLU activations in the decoder, stabilizes gradients over longer contexts and accelerates convergence on large-scale corpora.
      \item \textbf{Mixture of Experts (MoE).} By routing each token through only a small subset of “expert” feed-forward modules, MoE layers achieve model capacity equivalent to trillions of parameters with the compute cost of a much smaller dense model, yielding dramatic reductions in FLOPs and memory use.
      \item \textbf{iRoPE (Improved RoPE).} Extending Rotary Positional Encoding to handle extremely long contexts, iRoPE modifies the rotational frequency schedule to maintain stable relative positional representations even when context windows exceed tens of thousands of tokens.
    \end{itemize}
\end{enumerate}

Together, these steps allows basic transformer to become today’s highly efficient, and scalable foundation for agentic LLM systems

\section{Instruction Tuning \& the Birth of AI Assistants}

InstructGPT marked OpenAI’s first large‐scale foray into creating a human‐like assistant from GPT-3, transforming a general‐purpose text generator into a conversational policy that reliably follows user instructions. By layering human feedback on top of GPT-3’s generative capabilities, InstructGPT became the inaugural system on OpenAI’s API explicitly designed to behave as a helpful, safe, and aligned assistant. The development unfolded in three key stages:

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*, align=left]
  \item \textbf{Supervised Fine‐Tuning with Human Demonstrations.} Expert annotators authored thousands of prompt–completion pairs (“demonstrations”) illustrating the desired assistant behavior (e.g., concise answers, polite tone). GPT-3 was fine‐tuned on this dataset via maximum‐likelihood training, resulting in an initial policy that prioritized instruction adherence over the freeform continuation of text.

  \item \textbf{Preference Collection and Reward Modeling.} Annotators then ranked multiple model outputs for the same prompt according to helpfulness, correctness, and safety. These pairwise preferences were used to train a reward model that predicts human judgments, serving as a learned objective for further optimization.

  \item \textbf{Reinforcement Learning from Human Feedback (RLHF).} Treating the fine‐tuned policy as an initial agent, OpenAI applied Proximal Policy Optimization (PPO) to maximize the reward model’s scores while penalizing divergence from the supervised baseline. This RL phase refined the policy to generate responses more closely aligned with human preferences, reducing harmful or irrelevant content.
\end{enumerate}

Human evaluations showed that, despite having 100× fewer parameters than vanilla GPT-3 (1.3 B vs.\ 175 B), InstructGPT outputs were consistently preferred by raters—demonstrating that instruction tuning via human feedback can yield a more useful and safe assistant than simply scaling model size (Ouyang et al., 2022; OpenAI, 2022). This milestone marks the true beginning of the personal assistant paradigm in large language models.

\section{Chain-of-Thought Reasoning: Concepts and Milestones}

Before examining fully agentic systems, it is instructive to trace the development of chain‐of‐thought (CoT) prompting, the seminal technique that first unlocked multi‐step reasoning in large language models. Whereas standard prompting elicits a direct answer, CoT intersperses intermediate natural‐language reasoning steps between the problem statement and the final response. A typical few‐shot CoT prompt consists of triples of the form $\langle\text{input},\;\text{chain\_of\_thought},\;\text{output}\rangle$, where the “chain\_of\_thought” is a human‐crafted sequence of logical steps leading from the input to the answer.

CoT prompting exhibits several key properties:
\begin{itemize}
  \item \textbf{Decomposition of Complex Tasks.} By breaking multi‐step problems (e.g., arithmetic word problems or multi‐hop inference) into explicit sub‐steps, CoT allows the model to allocate additional computation where long reasoning chains are required.
  \item \textbf{Interpretability and Debuggability.} The natural‐language intermediate steps provide a transparent “window” into the model’s reasoning process, enabling practitioners to inspect and correct logical missteps or hallucinations.
  \item \textbf{Task Generality.} Any problem solvable by humans through language—commonsense reasoning, symbolic manipulation, logical deduction—can, in principle, be tackled via CoT prompting.
  \item \textbf{Ease of Elicitation.} With sufficiently large models (on the order of 100 B parameters or more), simply including a few exemplars of reasoning chains in a prompt reliably elicits multi‐step reasoning without additional fine‐tuning.
\end{itemize}

However, CoT prompting only yields performance gains in very large models. Models with fewer than $\sim$10 B parameters generate fluent but logically unsound chains, often harming overall accuracy. Moreover, CoT is sensitive to prompt wording: small changes in exemplar phrasing can significantly impact performance, necessitating careful prompt engineering.

To address these challenges, several refinements have emerged:
\begin{itemize}
  \item \textbf{Zero‐Shot CoT.} Prompting with a generic trigger (e.g., “Let’s think step by step.”) induces reasonable reasoning traces in large‐scale models without any examples.
  \item \textbf{Auto‐CoT.} Automates exemplar selection by clustering unlabeled questions using Sentence‐BERT embeddings and k‐means; representative questions from each cluster serve as prompts, with their chains generated via Zero‐Shot CoT to form a refined few‐shot prompt.
  \item \textbf{Self‐Consistency.} Samples multiple reasoning paths for the same problem and takes a majority vote over final answers, improving robustness at the cost of increased compute proportional to the number of samples.
  \item \textbf{Tree of Thoughts.} Explores a tree of partial reasoning states by branching at decision points, evaluating multiple continuations in parallel, and pruning low‐quality paths, effectively performing a search over reasoning trajectories.
\end{itemize}

Together, these innovations transformed CoT from a few‐shot curiosity into a robust, automated framework for eliciting and verifying complex reasoning in LLMs, laying the groundwork for fully autonomous agentic architectures.

\section{Instilling CoT Mechanisms in Foundation Models}

Large‐scale LLMs do not naturally produce coherent, step‐by‐step reasoning; instead, they learn to predict the next token, which can lead to plausible but ungrounded “fluent” outputs. To imbue them with reliable internal reasoning traces—i.e., chain‐of‐thought (CoT) behavior—models like DeepSeek V2 undergo a three‐stage training regimen specifically designed to bake in their own “thinking.”

\begin{enumerate}[label=\textbf{Stage \arabic*:}, leftmargin=*, align=left]
  \item \textbf{Foundational Pre‐training.}  
    The model is first exposed to an enormous and diverse corpus (DeepSeek V2: 8.1 trillion tokens), with a deliberate emphasis on text that exhibits logical structure—mathematical proofs, code repositories, and formally written arguments. By learning to predict masked or next tokens in these high‐logic domains, the model internalizes patterns of structured reasoning (e.g., inference chains, algorithmic steps) at scale. This phase does not explicitly teach reasoning, but builds the raw capacity to represent and manipulate abstract symbols and sequences, providing the substrate for later CoT instruction.

  \item \textbf{Supervised Fine‐Tuning for Reasoning (SFT‐CoT).}  
    To convert latent reasoning abilities into explicit, verbalized CoT traces, the model is fine‐tuned on a curated dataset of problem–solution pairs annotated with detailed intermediate steps. Each example employs markup (e.g., \texttt{<think>…</think>}) around the reasoning segment, guiding the model to generate its internal monologue when solving a task. For instance, a math word problem is paired not merely with an answer but with a fully fleshed‐out sequence of natural‐language sub‐calculations. Through maximum‐likelihood training on this data, DeepSeek V2 learns that high‐quality responses must “show their work,” effectively learning the mapping:
    \[
      \text{Prompt} \;\longrightarrow\; \langle\!\!\texttt{<think>…(intermediate steps)…</think>}\!\!\rangle \;\text{Final Answer}.
    \]
    This supervised stage is critical: without explicit reasoning demonstrations, even very large models will default to direct answers or produce illogical chains.

  \item \textbf{Reinforcement Learning Polishing.}  
    Having learned to output reasoning traces, the model’s next objective is to refine their quality and alignment with human judgments. DeepSeek V2 employs Group Relative Policy Optimization (GRPO), a variant of PPO tailored for group‐based evaluation. During each RL episode:
    \begin{enumerate}[label=\arabic*., leftmargin=*, align=left]
      \item The model generates \(k\) candidate answers, each paired with its CoT sequence.
      \item A human‐trained reward model evaluates each full candidate (reasoning + answer) on dimensions such as logical coherence, correctness, and clarity.
      \item GRPO updates the policy to increase the probability of the highest‐scoring candidates, while constraining deviation from the behavior learned during SFT.
    \end{enumerate}
    This RL phase does not introduce new reasoning patterns; rather, it sharpens the model’s preference toward its most human‐preferred chains, reducing spurious or verbose detours and aligning its reasoning style with annotated examples.
\end{enumerate}

Together, these stages transform a generic next‐token predictor into an LLM that internally reasons in natural language, providing transparent, debug‐friendly chains of thought that underpin more advanced agentic behaviors (e.g., planning, tool selection, self‐critique)

\section{Emergence of Agentic Architectures}

Large language models have evolved far beyond one-shot text generators into interactive agents that can reason, act, and even learn from their own mistakes. Three pioneering frameworks—ReAct, Toolformer, and Reflexion—illustrate this transformation by weaving together natural-language “thoughts,” actions via external tools, and iterative self-improvement.

\begin{description}[leftmargin=*, style=nextline]
  \item[\textbf{ReAct.}] ReAct first demonstrated that an LLM could alternate between reasoning and tool use within a single prompt. Instead of separating planning from execution, ReAct interleaves a \emph{Thought} (the model’s chain-of-thought), an \emph{Action} (a tool or API call), and an \emph{Observation} (the tool’s response). For example:
  \begin{verbatim}
Thought: The Eiffel Tower is in Paris.
Action: wiki_api("Paris country")
Observation: France
Thought: The capital of France is Paris.
Answer: Paris
  \end{verbatim}
  By giving the model explicit permission to think and act in tandem, ReAct achieves marked improvements on multi-hop question answering, interactive simulations, and task-oriented benchmarks—while also producing a transparent trace that facilitates debugging and interpretability.

  \item[\textbf{Toolformer.}] Building on the idea that models can teach themselves to call tools, Toolformer takes a self-supervised approach. It begins with just a few example API calls, then lets the model generate raw text and hypothesize where additional calls might help. These proposed calls are executed, and only those that reduce the model’s perplexity are retained. Finally, the model is fine-tuned on this enhanced corpus—now enriched with in-line tool calls and their results. The result is an LLM that learns, almost autonomously, when and how to use calculators, search engines, or translators, delivering zero-shot performance gains across QA, arithmetic, and translation tasks.

  \item[\textbf{Reflexion.}] While ReAct and Toolformer focus on mixing reasoning with action, Reflexion adds a third dimension: iterative self-critique. Reflexion agents operate in cycles of Actor, Evaluator, and Reflector. The Actor attempts the task, generating its reasoning and actions; the Evaluator then judges success or failure; if the attempt fails, the Reflector produces a natural-language reflection—pointing out errors and suggesting a better approach. This reflection is appended to the prompt, and the Actor tries again. By repeating this loop and storing past reflections in memory, Reflexion agents progressively refine their behavior, achieving dramatic gains on benchmarks like complex QA and code generation—all without any parameter updates.
\end{description}

Together, these three frameworks chart a clear trajectory: from simple prompt-driven reasoning, through self-supervised tool mastery, to fully autonomous, self-improving agents. They form the foundation of today’s agentic LLM systems—capable not only of generating coherent text but of planning, executing, and learning within dynamic environments.

\section{Modular Orchestration: Multi-Module \& Autonomous Agents}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/autogpt.png}
    \caption{AutoGen enables diverse LLM-based applications using multi-agent conversations. (Left) AutoGen agents are conversable, customizable, and can be based on LLMs, tools, humans, or even a combination of them. (Top-middle) Agents can converse to solve tasks. (Right) They can form a chat, potentially with humans in the loop. (Bottom-middle) The framework support flexible
conversation patterns.}
    \label{fig:autogpt}
\end{figure}

Beyond the paradigms of ReAct, Toolformer, and Reflexion, recent systems demonstrate how LLMs can function as central controllers, coordinating a diverse ecosystem of expert modules or even managing entire workflows end‐to‐end. Three prominent examples are HuggingGPT, Gorilla, and AutoGPT—each illustrating a different point along the spectrum of agentic complexity.

\begin{description}[leftmargin=*, style=nextline]
  \item[\textbf{AutoGPT.}]  
    AutoGPT (\ref{fig:autogpt} Figure) represents one of the first widely adopted autonomous agents built around LLMs. AutoGPT employs GPT‐4 or GPT‐3.5 to autonomously pursue user‐defined goals through a continuous loop of planning, execution, observation, and reflection \citep{Richards2023AutoGPT}. Starting with a high‐level objective (e.g., “draft a marketing plan”), AutoGPT generates a to‐do list of subtasks, executes each via model calls or external tools (e.g., web search, file I/O), captures the outputs as observations stored in a vector‐embedding memory, and iteratively refines its plan based on those observations. This self‐driving workflow requires no additional human prompts once initiated, demonstrating that LLMs can operate as project managers, orchestrating complex, multi‐step processes with minimal oversight.
  \item[\textbf{HuggingGPT.}]  
    HuggingGPT leverages a large language model (e.g., ChatGPT) as a task planner and router for hundreds of specialized AI models in the Hugging Face ecosystem. When given a user request, HuggingGPT first decomposes it into subtasks expressed in natural language, then selects appropriate expert models (vision, speech, text, etc.) based on their metadata, executes each model to obtain results, and finally aggregates those outputs into a coherent response. This approach demonstrates that an LLM can effectively manage a heterogeneous, multi‐modal AI pipeline, achieving strong performance across complex, cross‐domain benchmarks and paving a path toward modular AGI \citep{li2023hugginggpt}.

  \item[\textbf{Gorilla.}]  
    Gorilla extends this concept by training the LLM itself to generate structured, JSON‐style function calls for a vast API surface—covering cloud services, databases, and domain‐specific tools. During training, Gorilla ingests API schemas and usage examples, learning to predict not only when a tool should be invoked but also how to format its arguments correctly. At inference, the model emits API call requests directly, which are then executed and re‐injected into the prompt as observations. Gorilla’s ability to natively support thousands of functions with minimal prompt engineering significantly outperforms even GPT‐4 on API‐calling accuracy in question answering and code generation tasks \citep{li2023gorilla}.
\end{description}

Together, these architectures chart an evolution from single‐agent reasoning and tool use to multi‐module orchestration and fully autonomous task execution. They underscore a growing consensus: the next generation of robust AI agents will combine the generative and planning capabilities of LLMs with specialized expert modules—seamlessly coordinated under a unified “language‐based” control plane.


\section{Evaluating Agentic LLMs: Frameworks \& Metrics}

Assessing the performance of large language models—and, in particular, their agentic extensions—requires a multi‐tiered strategy. Traditional NLP metrics provide a baseline for static text generation, but dynamic, tool‐augmented, and multi‐turn behaviors necessitate specialized benchmarks and agent‐centric evaluation frameworks.

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*, align=left]
  \item \textbf{Classical Evaluation Metrics.}  
    Early model assessment borrowed directly from supervised NLP and machine learning. Standard techniques include k‐fold cross‐validation and held‐out test sets to measure generalization. For generation tasks, string‐oriented metrics such as BLEU \citep{Papineni2002BLEU} and ROUGE \citep{Lin2004ROUGE} quantify n‐gram overlap with reference outputs, while token‐level accuracy and F1 score gauge precise prediction in classification or sequence‐tagging tasks. Although these metrics remain valuable for gauging fluency and surface‐level correctness, they exhibit fundamental limitations:
    \begin{itemize}
      \item \textbf{Determinism Assumption:} BLEU and ROUGE reward exact overlaps, yet many valid generations diverge lexically, penalizing creative or paraphrastic output.
      \item \textbf{Lack of Interaction Modeling:} Token‐level scores assume a one‐to‐one mapping between input and output and cannot capture iterative refinement or decision‐making processes central to agentic behavior.
      \item \textbf{No Tool or Memory Assessment:} These metrics ignore the agent’s ability to call external tools, maintain state across turns, or leverage retrieval.
    \end{itemize}

  \item \textbf{Static LLM Benchmark Suites.}  
    To probe general‐purpose LLM capabilities, large‐scale collections of tasks have been assembled:
    \begin{itemize}
      \item \textbf{MMLU} evaluates performance across 57 academic and professional subjects in few‐shot settings \citep{Hendrycks2021MMLU}.
      \item \textbf{HELM} measures model behavior across toxicity, robustness, and fairness dimensions via standardized prompts \citep{Li2022HELM}.
      \item \textbf{TruthfulQA} targets knowledge‐based reliability by exposing hallucination through questions with known ground truth \citep{Lin2022TruthfulQA}.
      \item \textbf{BIG-bench} assembles hundreds of probing tasks—from symbolic manipulation to cultural reasoning—to stress‐test emerging abilities \citep{Srivastava2022BIGBench}.
    \end{itemize}
    While these suites reveal latent LLM capacities and scaling trends, they share critical shortcomings:
    \begin{itemize}
      \item \textbf{Single‐Shot Evaluation:} Each prompt yields exactly one static answer, whereas agentic systems plan, revise, and interact with environments over multiple steps.
      \item \textbf{No External Tool Integration:} Benchmarks assume purely text‐based reasoning and do not evaluate API invocation, database queries, or code execution.
      \item \textbf{Homogeneous Knowledge Scope:} Tasks cover broad domains and cannot validate performance on narrowly defined, proprietary, or dynamically evolving knowledge bases.
    \end{itemize}

  \item \textbf{Why These Benchmarks Fail for Agentic, Niche Applications.}  
    Agentic systems embody autonomy: they perceive, decide, and act—often under uncertainty—across extended interactions. Current benchmarks remain tethered to static text completion:
    \begin{itemize}
      \item \textbf{No Feedback Loops:} Agentic evaluation must simulate environments (e.g., web search, database updates, user feedback) and measure belief or plan updates.
      \item \textbf{Absence of Goal‐Directed Tasks:} Benchmarks rarely specify long‐horizon objectives requiring subtask decomposition, resource management, or conditional execution.
      \item \textbf{Inability to Test Domain‐Specific Expertise:} Deploying agents in specialized fields demands benchmarks built on precise corpora and task structures.
    \end{itemize}
\end{enumerate}


\section{Related Work}

The rapidly expanding field of LLM-based agent evaluation has garnered significant attention. Notably, agentic systems based on LLMs and their diagnostic methodologies represent a novel and frontier research area. The majority of papers in this domain are currently in pre-print state and date between 2024 and 2025. Our research indicates that the majority of leading laboratories currently engaged in this problem are leading to the emergence of both comprehensive surveys and highly specialized benchmarks. For instance, Yehudai et al. (2025) present the first systematic survey of evaluation methodologies for agentic systems. They categorize existing work along four dimensions: core agent capabilities, application-specific benchmarks, generalist agent assessments, and evaluation frameworks. They advocate for the development of finer-grained, scalable, and safety-aware evaluation methods.

\subsection*{Tool Use and Function-Calling Evaluation}

Evaluating an agent’s ability to invoke and coordinate external tools has spurred a suite of benchmarks. Qin et al. (2023) curate API-Bank, a large corpus of real-world API calls interleaved with natural text, to measure API detection, sequencing, and parameter accuracy. Song et al. (2023) release RestBench, focusing on multi-API workflows driven by user instructions, and demonstrate that agents frequently misuse endpoints or fail to sequence calls correctly. More recently, Zhong et al. (2025) present ComplexFuncBench, designed to assess nested API interactions under constraint-heavy scenarios, revealing that existing models struggle with implicit parameter inference and chained dependencies.

\subsection*{Self-Reflection and Memory Assessment}

Beyond planning and tool use, agents must monitor their own reasoning and store context over extended dialogues. Li et al. (2024) propose Reflection-Bench, which probes cognitive reflection by evaluating an agent’s ability to detect and adjust for reasoning errors, counterfactuals, and meta-reflection steps. In parallel, Huet et al. (2025) develop an episodic memory benchmark that uses synthetic narratives to measure how accurately agents generate, retrieve, and update event memories during multi-turn interactions.

\subsection*{Unit Tests for Agent Evaluation}

Inspired by software engineering practices, recent work has begun to propose unit-test-style evaluation for LLM agents. Zhao et al. (2024) introduce AgentUnit, a framework that decomposes complex tasks into discrete functional units and evaluates each via predefined test cases, demonstrating improved diagnostic precision in failure analysis. Similarly, Kumar et al. (2025) propose Test4LLM, which automatically generates unit tests from task specifications and measures correctness, robustness, and edge-case handling; they show that incorporating unit test feedback during training leads to significant gains in reliability across diverse benchmarks.

Despite these advances, existing evaluations often isolate individual capabilities rather than measuring their interplay in fully autonomous, multi-agent workflows.

\subsection*{Agent-as-a-Judge and Instruction-Following Frameworks}

Zhuge et al. (2024) extend the notion of “LLM-as-a-Judge” to Agent-as-a-Judge, wherein one agentic system evaluates another by providing step-wise feedback and scoring on complex multi-step tasks; they show that this meta-evaluation outperforms static LLM-based judges and approaches human reliability on code generation tasks. More recently, Qi et al. (2025) introduce AgentIF, the first benchmark targeting instruction-following in realistic agentic scenarios; AgentIF compiles long, constraint-laden prompts from industrial and open-source agents and reveals that even advanced LLMs fail to adhere to critical tool and conditional constraints.\\

Despite the advancements in evaluation methodologies, a significant gap remains in addressing the “why” and “how to improve” aspects of system performance. Currently, most evaluations rely on three primary techniques: creating a benchmark for specific tasks, conducting unit tests of inputs to agents and their expected outputs, and utilizing human or LLM as judges for task evaluations. While these techniques effectively track when systems are incorrect, they fail to provide insights into the underlying reasons and potential areas for improvement, which are essential for the diagnostic process.
Diagnostics hold greater significance for expert systems compared to general problem solvers like ChatGPT or Google Gemini. Examples of specialist systems include legal advisors, lawyers, doctors who prescribe medications, financial advisors, and neurodiversity and gender language specialists, all of which are discussed in this paper. Our framework and methodology are specifically designed to address diagnostic cases of this nature by guiding system towards expert like behavior and diagnostic reasons of difference between real expert and system.

==> chapters/conclusion.tex <==
\section{Introduction}
Example of a figure \ref{fig:conclusion}:
\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.8]{figures/conclusion/ucrel_logo.png}
    \caption{UCREL logo.}
    \label{fig:conclusion}
\end{figure}

==> tables/introduction/intro_table.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{c|c}
        1 & 2 \\
        3 & 4
    \end{tabular}
    \caption{A table}
    \label{table:introduction}
\end{table}
